MLZero: A Multi-Agent System for End-to-end Machine Learning Automation

Existing AutoML systems have advanced the automation of machine learning (ML); however, they still require substantial manual configuration and expert input, particularly when handling multimodal data. We introduce MLZero, a novel multi-agent framework powered by Large Language Models (LLMs) that enables end-to-end ML automation across diverse data modalities with minimal human intervention. A cognitive perception module is first employed, transforming raw multimodal inputs into perceptual context that effectively guides the subsequent workflow. To address key limitations of LLMs, such as hallucinated code generation and outdated API knowledge, we enhance the iterative code generation process with semantic and episodic memory. MLZero demonstrates superior performance on MLE-Bench Lite, outperforming all competitors in both success rate and solution quality, securing six gold medals. Additionally, when evaluated on our Multimodal AutoML Agent Benchmark, which includes 25 more challenging tasks spanning diverse data modalities, MLZero outperforms the competing methods by a large margin with a success rate of 0.92 (+263.6\%) and an average rank of 2.28. Our approach maintains its robust effectiveness even with a compact 8B LLM, outperforming full-size systems from existing solutions.

==> assets/dataset_info.tex <==
\iffalse
\begin{table}[ht]
\centering
\small
\caption{Dataset information with modality and evaluation metrics}
\begin{tabular}{p{2cm}p{2.5cm}p{1.2cm}}
\toprule
\textbf{Dataset} & \textbf{Modality} & \textbf{Metric} \\
\midrule
Abalone & Tab & RMSE↓ \\
Airbnb & Tab & F1(weighted)↑ \\
Airlines & Tab & AUROC↑ \\
Bioresponse & Tab & AUROC↑ \\
Camo Seg & Img & $S_\alpha$↑ \\
CD18 & Img, Txt & $R^2$↑ \\
Climate Fvr & Txt & Recall@10↑ \\
Covertype & Tab & F1(weighted)↑ \\
Elec Hourly & Tab, Time & MASE↓ \\
EU Flood & Img & F1↑ \\
FiQA & Txt & Recall@10↑ \\
GNAD10 & Txt & F1(weighted)↑ \\
HAM10000 & Img & F1(weighted)↑ \\
HatefulMeme & Img, Txt & F1↑ \\
ISIC2017 & Img & IoU↑ \\
Funding & Tab, Txt & F1↑ \\
MEmotion & Img, Txt & Hamming Loss \\
MLDoc & Txt, Tab & F1(weighted)↑ \\
NN5 Daily & Tab, Time & MASE↓ \\
Petfinder & Img, Txt & F1(weighted)↑ \\
Road Seg & Img & IoU↑ \\
RVL-CDIP & Img & F1(weighted)↑ \\
Solar 10m & Tab, Time & MASE↓ \\
Clothing & Txt & $R^2$↑ \\
Yolanda & Img & RMSE↓ \\
\bottomrule
\end{tabular}
\label{tab:dataset_info}
\end{table}
\fi

\begin{table}[htbp]
\centering
\caption{Dataset Indices and MLE-Bench Information}
\label{tab:mlebench_dataset_info}
\begin{tabular}{clcccc}
\toprule
ID & Dataset Name & Gold & Silver & Bronze & Median \\
\midrule
D1 & Aerial Cactus Identification ($\uparrow$) & 1.0000 & 1.0000 & 1.0000 & 0.9991 \\
D2 & APTOS 2019 Blindness Detection ($\uparrow$) & 0.9305 & 0.9197 & 0.9145 & 0.8889 \\
D3 & Denoising Dirty Documents ($\downarrow$) & 0.0179 & 0.0261 & 0.0452 & 0.0733 \\
D4 & Detecting Insults in Social Commentary ($\uparrow$) & 0.8332 & 0.8231 & 0.7911 & 0.7784 \\
D5 & Dog Breed Identification ($\downarrow$) & 0.0005 & 0.0054 & 0.0460 & 0.4721 \\
D6 & Dogs vs Cats Redux ($\downarrow$) & 0.0388 & 0.0504 & 0.0613 & 0.1222 \\
D7 & Histopathologic Cancer Detection ($\uparrow$) & 0.9835 & 0.9798 & 0.9738 & 0.9477 \\
D8 & Jigsaw Toxic Comment Classification ($\uparrow$) & 0.9874 & 0.9867 & 0.9864 & 0.9808 \\
D9 & Leaf Classification ($\downarrow$) & 0.0000 & 0.0079 & 0.0153 & 0.1083 \\
D10 & MLSP 2013 Birds ($\uparrow$) & 0.9353 & 0.9004 & 0.8737 & 0.8657 \\
D11 & NYC Taxi Fare Prediction ($\downarrow$) & 2.8338 & 2.8819 & 2.9237 & 3.5974 \\
D12 & NOMAD 2018 Conductors ($\downarrow$) & 0.0559 & 0.0623 & 0.0658 & 0.0699 \\
D13 & Plant Pathology 2020 FGVC7 ($\uparrow$) & 0.9784 & 0.9747 & 0.9736 & 0.9485 \\
D14 & Random Acts of Pizza ($\uparrow$) & 0.9791 & 0.7648 & 0.6921 & 0.5996 \\
D15 & SIIM-ISIC Melanoma Classification ($\uparrow$) & 0.9455 & 0.9401 & 0.9370 & 0.9128 \\
D16 & Spooky Author Identification ($\downarrow$) & 0.1651 & 0.2700 & 0.2938 & 0.4188 \\
D17 & Tabular Playground Dec 2021 ($\uparrow$) & 0.9566 & 0.9566 & 0.9566 & 0.9534 \\
D18 & Tabular Playground May 2022 ($\uparrow$) & 0.9982 & 0.9982 & 0.9982 & 0.9727 \\
D19 & Text Normalization English ($\uparrow$) & 0.9972 & 0.9914 & 0.9904 & 0.9904 \\
D20 & Text Normalization Russian ($\uparrow$) & 0.9901 & 0.9823 & 0.9759 & 0.9759 \\
D21 & ICML 2013 Whale Challenge ($\uparrow$) & 0.9896 & 0.9502 & 0.9052 & 0.8652 \\
\bottomrule
\end{tabular}
\end{table}

==> assets/main_results_backup_before_reorder.tex <==
\begin{table}[ht]
\centering
\small
\caption{Performance comparison across ML agents and $^{\star}$ablation configurations on Multimodal AutoML Agent Benchmark. Colorful icons indicate data modality (\texticon: text, \tabularicon: tabular, \imageicon: image, \docicon: document) and problem type (\binclassicon: binary classification, \multiclassicon: multiclass classification, \regressicon: regression, \forecasticon: forecasting, \segmenticon: semantic segmentation, \retrievalicon: retrieval, \multilabelicon: Multi Label Classification). $\uparrow$($\downarrow$) indicates higher(lower) is better. $^\dagger$Dagger columns are not agents, including \modelname's optimal performance with current ML libraries to compare with human performance reported in recent open sourced literature. \textbf{Bold} numbers indicates best ML agent performance with comparable \textbf{def}ault configurations. For each dataset, results are reported as mean\textsubscript{\textcolor{gray}{std}} format across three independent runs. Configuration descriptions: \textbf{def}: default settings of each agent, \textbf{8B$^*$}: using LLama 3.1 8B~\cite{llama3}, \textbf{-ext$^*$}: without external knowledge, \textbf{-epi$^*$}: without episodic memory, \textbf{+rea$^*$}: with reasoning LLM~\cite{o4mini}, \textbf{+ext$^*$}: with external knowledge. Performance metrics (Appendix~\ref{app:main_result_metrics_def}) are computed across three runs: \textbf{Avg. Rank}: average position when ranking agents by their mean valid performance on each dataset, \textbf{Rel. Time}: relative execution time compared to \modelname (def), \textbf{Success}: percentage of successful runs. Detailed results for each run and each agent are shown in Appendix~\ref{app:maab_result_details}.}
\setlength{\tabcolsep}{3.5pt}
\scalebox{0.75}{
\begin{tabular}{p{3cm}|*{5}{>{\centering\arraybackslash}p{1.1cm}@{}}|*{2}{>{\centering\arraybackslash}p{1.05cm}@{}}|*{2}{>{\centering\arraybackslash}p{1.05cm}@{}}|*{2}{>{\centering\arraybackslash}p{1.05cm}@{}}|>{\centering\arraybackslash}p{1.05cm}@{}|>{\centering\arraybackslash}p{1.5cm}}
\toprule
 \hspace{2cm}\textbf{Agent} & \multicolumn{5}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{}} & \textbf{} & \textbf{} \\
 & \multicolumn{5}{c|}{\textbf{\modelname (ours)}} & \multicolumn{2}{c|}{\textbf{Codex CLI}} & \multicolumn{2}{c|}{\textbf{AIDE}} & \multicolumn{2}{c|}{\textbf{DS-Agent}} & \textbf{AK} & \textbf{Human} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14}
\textbf{Dataset} & \textbf{def} & \textbf{8B$^*$} & \textbf{-ext$^*$} & \textbf{-epi$^*$} & \textbf{24hrs$^\dagger$} & \textbf{def} & \textbf{+rea$^*$} & \textbf{def} & \textbf{+ext$^*$} & \textbf{def} & \textbf{zero-shot} & \textbf{def} & \textbf{Reported$^\dagger$} \\
\midrule
abalone \tabularicon\regressicon$\downarrow$ & $\textbf{2.13}_{\textcolor{gray}{.01}}$ & $2.09_{\textcolor{gray}{.00}}$ & $2.19_{\textcolor{gray}{.02}}$ & $2.13_{\textcolor{gray}{.01}}$ & $2.08$ & $2.23_{\textcolor{gray}{.00}}$ & $2.27_{\textcolor{gray}{.06}}$ & $2.16_{\textcolor{gray}{.04}}$ & $2.18_{\textcolor{gray}{.04}}$ & $2.24_{\textcolor{gray}{.00}}$ & $2.36_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ \\
airbnb \texticon\tabularicon\multiclassicon$\uparrow$ & $\textbf{0.43}_{\textcolor{gray}{.00}}$ & $0.42_{\textcolor{gray}{.01}}$ & $0.24_{\textcolor{gray}{.16}}$ & $0.42_{\textcolor{gray}{.01}}$ & $0.45$ & $\times$ & $0.39_{\textcolor{gray}{.00}}$ & $0.39_{\textcolor{gray}{.00}}$ & $0.39_{\textcolor{gray}{.03}}$ & $\times$ & $0.31_{\textcolor{gray}{.00}}$ & $0.32_{\textcolor{gray}{.05}}$ & $\times$ \\
airlines \tabularicon\binclassicon$\uparrow$ & $\textbf{0.66}_{\textcolor{gray}{.00}}$ & $0.69_{\textcolor{gray}{.04}}$ & $0.63_{\textcolor{gray}{.01}}$ & $0.66_{\textcolor{gray}{.00}}$ & $0.66$ & $\times$ & $0.63_{\textcolor{gray}{.02}}$ & $\times$ & $0.65_{\textcolor{gray}{.01}}$ & $\times$ & $0.61_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ \\
bio \tabularicon\binclassicon$\uparrow$ & $0.81_{\textcolor{gray}{.01}}$ & $0.80_{\textcolor{gray}{.00}}$ & $0.83_{\textcolor{gray}{.04}}$ & $0.80_{\textcolor{gray}{.00}}$ & $0.82$ & $0.79_{\textcolor{gray}{.00}}$ & $0.85_{\textcolor{gray}{.04}}$ & $\textbf{0.87}_{\textcolor{gray}{.00}}$ & $0.84_{\textcolor{gray}{.04}}$ & $0.79_{\textcolor{gray}{.00}}$ & $0.79_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ \\
camoseg \imageicon\segmenticon$\uparrow$ & $\textbf{0.84}_{\textcolor{gray}{.00}}$ & $\times$ & $0.46_{\textcolor{gray}{.00}}$ & $0.84_{\textcolor{gray}{.00}}$ & $0.85$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $0.89$ \\
cd18 \imageicon\tabularicon\regressicon$\uparrow$ & $\textbf{0.46}_{\textcolor{gray}{.02}}$ & -$0.21_{\textcolor{gray}{.65}}$ & -$1.57_{\textcolor{gray}{1.85}}$ & $0.51_{\textcolor{gray}{.06}}$ & $0.15$ & -$0.94_{\textcolor{gray}{.53}}$ & -$1.44_{\textcolor{gray}{.17}}$ & $\times$ & -$0.05_{\textcolor{gray}{.29}}$ & -$1.94_{\textcolor{gray}{.00}}$ & -$0.64_{\textcolor{gray}{.98}}$ & -$1.84_{\textcolor{gray}{.00}}$ & $\times$ \\
climate \texticon\retrievalicon$\uparrow$ & $\textbf{0.48}_{\textcolor{gray}{.00}}$ & $\times$ & $0.24_{\textcolor{gray}{.01}}$ & $0.48_{\textcolor{gray}{.00}}$ & $0.48$ & $\times$ & $0.20_{\textcolor{gray}{.05}}$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
covertype \tabularicon\multiclassicon$\uparrow$ & $\textbf{0.98}_{\textcolor{gray}{.00}}$ & $0.98_{\textcolor{gray}{.00}}$ & $0.88_{\textcolor{gray}{.01}}$ & $0.98_{\textcolor{gray}{.00}}$ & $0.98$ & $0.96_{\textcolor{gray}{.00}}$ & $0.92_{\textcolor{gray}{.05}}$ & $0.88_{\textcolor{gray}{.00}}$ & $0.86_{\textcolor{gray}{.09}}$ & $0.96_{\textcolor{gray}{.00}}$ & $0.95_{\textcolor{gray}{.00}}$ & $0.94_{\textcolor{gray}{.00}}$ & $\times$ \\
electric(H) \tabularicon\forecasticon$\downarrow$ & $\textbf{1.42}_{\textcolor{gray}{.02}}$ & $\times$ & $1.75_{\textcolor{gray}{.00}}$ & $1.40_{\textcolor{gray}{.01}}$ & $1.30$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $11.66_{\textcolor{gray}{.00}}$ & $\times$ & $1.23$ \\
flood \imageicon\binclassicon$\uparrow$ & $0.69_{\textcolor{gray}{.00}}$ & $0.69_{\textcolor{gray}{.00}}$ & $0.60_{\textcolor{gray}{.09}}$ & $0.68_{\textcolor{gray}{.00}}$ & $0.80$ & $\times$ & $0.44_{\textcolor{gray}{.00}}$ & $\textbf{0.71}_{\textcolor{gray}{.01}}$ & $0.68_{\textcolor{gray}{.02}}$ & $\times$ & $\times$ & $0.58_{\textcolor{gray}{.00}}$ & $0.79$ \\
fiqa \texticon\retrievalicon$\uparrow$ & $\textbf{0.50}_{\textcolor{gray}{.01}}$ & $\times$ & $0.22_{\textcolor{gray}{.00}}$ & $0.46_{\textcolor{gray}{.06}}$ & $0.48$ & $\times$ & $0.20_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $0.78$ \\
gnad10 \texticon\multiclassicon$\uparrow$ & $0.86_{\textcolor{gray}{.04}}$ & $0.85_{\textcolor{gray}{.00}}$ & $0.88_{\textcolor{gray}{.01}}$ & $0.83_{\textcolor{gray}{.00}}$ & $0.89$ & $0.82_{\textcolor{gray}{.03}}$ & $0.85_{\textcolor{gray}{.00}}$ & $\textbf{0.90}_{\textcolor{gray}{.01}}$ & $0.58_{\textcolor{gray}{.00}}$ & $\times$ & $0.80_{\textcolor{gray}{.11}}$ & $0.11_{\textcolor{gray}{.00}}$ & $0.90$ \\
ham10000 \imageicon\tabularicon\multiclassicon$\uparrow$ & $0.63_{\textcolor{gray}{.11}}$ & $0.57_{\textcolor{gray}{.00}}$ & $0.67_{\textcolor{gray}{.00}}$ & $0.67_{\textcolor{gray}{.11}}$ & $0.56$ & $0.48_{\textcolor{gray}{.00}}$ & $0.47_{\textcolor{gray}{.03}}$ & $\textbf{0.81}_{\textcolor{gray}{.00}}$ & $0.81_{\textcolor{gray}{.03}}$ & $\times$ & $\times$ & $\times$ & $0.61$ \\
hateful \texticon\imageicon\binclassicon$\uparrow$ & $\textbf{0.59}_{\textcolor{gray}{.01}}$ & $0.57_{\textcolor{gray}{.04}}$ & $0.35_{\textcolor{gray}{.04}}$ & $0.59_{\textcolor{gray}{.01}}$ & $0.61$ & $\times$ & $0.48_{\textcolor{gray}{.07}}$ & $0.51_{\textcolor{gray}{.05}}$ & $0.49_{\textcolor{gray}{.03}}$ & $\times$ & $\times$ & $0.36_{\textcolor{gray}{.02}}$ & $0.60$ \\
isic2017 \imageicon\segmenticon$\uparrow$ & $\textbf{0.75}_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ & $0.76$ & $\times$ & $0.11_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $0.78$ \\
funding \texticon\tabularicon\binclassicon$\uparrow$ & $\textbf{0.45}_{\textcolor{gray}{.02}}$ & $0.41_{\textcolor{gray}{.06}}$ & $0.36_{\textcolor{gray}{.06}}$ & $0.44_{\textcolor{gray}{.00}}$ & $0.51$ & $\times$ & $0.34_{\textcolor{gray}{.04}}$ & $\times$ & $0.44_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $0.24_{\textcolor{gray}{.00}}$ & $0.61$ \\
memotion \scalebox{0.8}{\texticon\imageicon\tabularicon\multilabelicon}$\uparrow$ & $0.50_{\textcolor{gray}{.01}}$ & $\times$ & $0.83_{\textcolor{gray}{.17}}$ & $0.51_{\textcolor{gray}{.00}}$ & $0.56$ & $\textbf{0.53}_{\textcolor{gray}{.00}}$ & $0.76_{\textcolor{gray}{.06}}$ & $0.47_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
mldoc \texticon\multiclassicon$\uparrow$ & $0.95_{\textcolor{gray}{.00}}$ & $0.95_{\textcolor{gray}{.00}}$ & $0.94_{\textcolor{gray}{.02}}$ & $0.95_{\textcolor{gray}{.00}}$ & $0.97$ & $0.32_{\textcolor{gray}{.23}}$ & $0.82_{\textcolor{gray}{.08}}$ & $\textbf{0.96}_{\textcolor{gray}{.00}}$ & $0.94_{\textcolor{gray}{.01}}$ & $0.95_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ \\
nn5(D) \tabularicon\forecasticon$\downarrow$ & $\textbf{0.76}_{\textcolor{gray}{.00}}$ & $\times$ & $1.14_{\textcolor{gray}{.32}}$ & $0.76_{\textcolor{gray}{.00}}$ & $0.79$ & $\times$ & $\times$ & $\times$ & $\times$ & $4.68_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $0.76$ \\
petfinder\scalebox{0.9}{\texticon\imageicon\tabularicon\multiclassicon}$\uparrow$ & $\textbf{0.39}_{\textcolor{gray}{.00}}$ & $0.40_{\textcolor{gray}{.01}}$ & $0.38_{\textcolor{gray}{.02}}$ & $0.39_{\textcolor{gray}{.00}}$ & $0.41$ & $\times$ & $0.40_{\textcolor{gray}{.00}}$ & $0.34_{\textcolor{gray}{.00}}$ & $0.38_{\textcolor{gray}{.01}}$ & $0.36_{\textcolor{gray}{.01}}$ & $0.27_{\textcolor{gray}{.08}}$ & $0.39_{\textcolor{gray}{.00}}$ & $0.41$ \\
roadseg \imageicon\segmenticon$\uparrow$ & $\textbf{0.47}_{\textcolor{gray}{.00}}$ & $\times$ & $0.31_{\textcolor{gray}{.13}}$ & $0.60_{\textcolor{gray}{.00}}$ & $0.47$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $0.62$ \\
rvlcdip \docicon\multiclassicon$\uparrow$ & $\textbf{0.87}_{\textcolor{gray}{.00}}$ & $\times$ & $0.89_{\textcolor{gray}{.00}}$ & $0.87_{\textcolor{gray}{.00}}$ & $0.92$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $0.96$ \\
solar(10m) \tabularicon\forecasticon$\downarrow$ & $1.49_{\textcolor{gray}{.78}}$ & $\times$ & $\times$ & $1.29_{\textcolor{gray}{.00}}$ & $0.18$ & $\times$ & $1.29_{\textcolor{gray}{.00}}$ & $\textbf{1.05}_{\textcolor{gray}{.00}}$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
clothing \texticon\tabularicon\regressicon$\uparrow$ & $\textbf{0.75}_{\textcolor{gray}{.00}}$ & $0.61_{\textcolor{gray}{.11}}$ & $0.66_{\textcolor{gray}{.03}}$ & $0.72_{\textcolor{gray}{.04}}$ & $0.77$ & $\times$ & $0.35_{\textcolor{gray}{.23}}$ & $\times$ & $0.75_{\textcolor{gray}{.00}}$ & $\times$ & $0.35_{\textcolor{gray}{.00}}$ & $\times$ & $0.74$ \\
yolanda \tabularicon\regressicon$\downarrow$ & $\textbf{8.53}_{\textcolor{gray}{.00}}$ & $8.54_{\textcolor{gray}{.00}}$ & $8.93_{\textcolor{gray}{.03}}$ & $8.53_{\textcolor{gray}{.00}}$ & $8.18$ & $\times$ & $9.43_{\textcolor{gray}{.24}}$ & $\times$ & $8.79_{\textcolor{gray}{.25}}$ & $\times$ & $\times$ & $\times$ & $\times$ \\
\midrule
\rowcolor{lightgray}
\textbf{Avg. Rank}$\downarrow$ & $\textbf{2.42}$ & $\textbf{5.14}$ & $\textbf{4.94}$ & $\textbf{2.86}$ & $\textbf{N/A}$ & $\textbf{8.04}$ & $\textbf{5.76}$ & $\textbf{6.16}$ & $\textbf{6.02}$ & $\textbf{8.26}$ & $\textbf{8.12}$ & $\textbf{8.28}$ & $\textbf{N/A}$ \\
\rowcolor{lightgray}
\textbf{Rel. Time}$\downarrow$ & $\textbf{1.0}$ & $\textbf{3.17}$ & $\textbf{2.32}$ & $\textbf{1.03}$ & $\textbf{N/A}$ & $\textbf{0.15}$ & $\textbf{0.23}$ & $\textbf{2.83}$ & $\textbf{2.48}$ & $\textbf{N/A}$ & $\textbf{N/A}$ & $\textbf{4.82}$ & $\textbf{N/A}$ \\
\rowcolor{lightgray}
\textbf{Success}$\uparrow$ & $\textbf{92.0\%}$ & $\textbf{45.3\%}$ & $\textbf{69.3\%}$ & $\textbf{86.7\%}$ & $\textbf{N/A}$ & $\textbf{14.7\%}$ & $\textbf{69.3\%}$ & $\textbf{25.3\%}$ & $\textbf{45.3\%}$ & $\textbf{13.3\%}$ & $\textbf{20.0\%}$ & $\textbf{14.7\%}$ & $\textbf{N/A}$ \\
\bottomrule
\end{tabular}
}
\vspace{-8mm}
\label{tab:main_results}
\end{table}

==> assets/main_results_detail.tex <==

\begin{table}[ht]
\centering
\small
\caption{Performance comparison across models and systems. Results are shown as ``metric value, execution time in seconds''. \ding{55} indicates failure or no result available.}
\scalebox{0.75}{
\begin{tabular}{p{1.8cm}*{6}{>{\centering\arraybackslash}p{2.1cm}}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{Ours}} & \multicolumn{3}{c}{\textbf{AIDE (w/ EXT.)}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \textbf{Claude 3.7 Sonnet} & \textbf{GPT-4o} & \textbf{o3-mini} & \textbf{Claude 3.7 Sonnet} & \textbf{GPT-4o} & \textbf{o3-mini} \\
\midrule
Abalone↓ & 2.13, 142 & 2.13, 105 & 2.13, 433 & 2.19, 385 & 2.75, 701 & \\
Airbnb↑ & 0.43, 1202 & 0.43, 2948 & 0.42, 3702 & 0.42, 2689 & \ding{55} & \\
Airlines↑ & 0.66, 1285 & 0.66, 1211 & 0.66, 4872 & \ding{55} & 0.63, 3608 & \\
Bioresponse↑ & 0.80, 3050 & 0.80, 302 & 0.80, 190 & 0.88, 7400 & 0.80, 359 & \\
Camo Seg↑ & 0.83, 4089 & 0.82, 1983 & 0.83, 2161 & \ding{55} & \ding{55} & \\
CD18↑ & 0.45, 215 & 0.45, 127 & 0.59, 2424 & 0.24, 248 & 0.53, 1734 & \\
Climate Fvr↑ & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
Covertype↑ & 0.98, 1963 & 0.98, 1934 & 0.98, 1982 & 0.74, 7856 & 0.98, 3613 & \\
Elec Hourly↓ & 1.44, 875 & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
EU Flood↑ & 0.68, 524 & 0.68, 985 & 0.68, 2495 & 0.70, 730 & 0.67, 3610 & \\
FiQA↑ & 0.48, 370 & \ding{55} & 0.48, 699 & \ding{55} & \ding{55} & \\
GNAD10↑ & 0.84, 717 & 0.84, 587 & 0.84, 3055 & \ding{55} & \ding{55} & \\
HAM10000↑ & 0.56, 815 & 0.56, 640 & 0.78, 3299 & 0.78, 813 & 0.57, 3613 & \\
HatefulMeme↑ & 0.57, 682 & 0.58, 481 & 0.57, 639 & 0.52, 2045 & 0.54, 3613 & \\
ISIC2017↑ & 0.75, 4139 & 0.76, 7423 & 0.74, 6660 & \ding{55} & \ding{55} & \\
Funding↑ & 0.44, 1330 & 0.44, 778 & 0.44, 839 & 0.44, 7496 & 0.44, 3613 & \\
MEmotion↑ & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
MLDoc↑ & 0.96, 3699 & 0.95, 261 & 0.94, 5409 & \ding{55} & 0.95, 1164 & \\
NN5 Daily↓ & 0.77, 251 & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
Petfinder↑ & 0.39, 701 & 0.38, 610 & 0.44, 1558 & 0.38, 2359 & \ding{55} & \\
Road Seg↑ & 0.47, 2069 & 0.47, 2809 & 0.49, 5903 & \ding{55} & \ding{55} & \\
RVL-CDIP↑ & 0.87, 2979 & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
Solar 10m↓ & 2.27, 800 & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \\
Clothing↑ & 0.75, 958 & 0.71, 4061 & 0.67, 4670 & 0.75, 1134 & \ding{55} & \\
Yolanda↓ & 8.53, 2066 & 8.53, 1868 & 8.53, 9274 & 8.54, 1953 & \ding{55} & \\
\bottomrule
\end{tabular}
}
\label{tab:performance_comparison}
\end{table}


\begin{table}[ht]
\centering
\small
\caption{Performance comparison across different methodologies. Results are shown as ``metric value, execution time in seconds''. \ding{55} indicates failure or no result available.}
\scalebox{0.75}{
\begin{tabular}{p{1.8cm}*{6}{>{\centering\arraybackslash}p{2.1cm}}}
\toprule
\textbf{Dataset} & \multicolumn{3}{c}{\textbf{AIDE}} & \textbf{DS-Agent} & \textbf{AutoKaggle} & \textbf{PlaceHolder} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}
& \textbf{Claude 3.7 Sonnet} & \textbf{GPT-4o} & \textbf{o3-mini} & \textbf{o3-mini} & \textbf{o3-mini} & \textbf{o3-mini} \\
\midrule
Abalone↓ & & 2.31, 68 & 2.23, 173 & & & \\
Airbnb↑ & & 0.63, 240 & \ding{55} & & & \\
Airlines↑ & & \ding{55} & \ding{55} & & & \\
Bioresponse↑ & & \ding{55} & \ding{55} & & & \\
Camo Seg↑ & & \ding{55} & \ding{55} & & & \\
CD18↑ & & \ding{55} & 0.68, 131 & & & \\
Climate Fvr↑ & & \ding{55} & \ding{55} & & & \\
Covertype↑ & & \ding{55} & \ding{55} & & & \\
Elec Hourly↓ & & \ding{55} & \ding{55} & & & \\
EU Flood↑ & & \ding{55} & \ding{55} & & & \\
FiQA↑ & & 0.75, 582 & \ding{55} & & & \\
GNAD10↑ & & \ding{55} & 0.88, 151 & & & \\
HAM10000↑ & & \ding{55} & 0.55, 209 & & & \\
HatefulMeme↑ & & 0.36, 3390 & 0.42, 518 & & & \\
ISIC2017↑ & & \ding{55} & \ding{55} & & & \\
Funding↑ & & \ding{55} & \ding{55} & & & \\
MEmotion↑ & & \ding{55} & \ding{55} & & & \\
MLDoc↑ & & 0.38, 144 & 0.87, 1769 & & & \\
NN5 Daily↓ & & \ding{55} & \ding{55} & & & \\
Petfinder↑ & & \ding{55} & \ding{55} & & & \\
Road Seg↑ & & \ding{55} & \ding{55} & & & \\
RVL-CDIP↑ & & \ding{55} & \ding{55} & & & \\
Solar 10m↓ & & \ding{55} & \ding{55} & & & \\
Clothing↑ & & \ding{55} & \ding{55} & & & \\
Yolanda↓ & & \ding{55} & 9.21, 4515 & & & \\
\bottomrule
\end{tabular}
}
\label{tab:methodology_comparison}
\end{table}

==> assets/more_llm.tex <==
\section{\modelname with more LLM Models}
\label{sec:more_llm}

We further evaluate the performance of other LLMs in \modelname:
\begin{itemize}
    \item \textbf{Default, Claude 3.7 Sonnet)}: Our primary system configuration.
    \item \textbf{DeepSeek R1}: 607B.
    \item \textbf{Claude 3.5 Haiku (claude-3-5-haiku-20241022)}: The smaller Claude.
    \item \textbf{Llama 3.3 70B}: 70B.
    \item \textbf{Llama 3.1 8B}: 8B.
\end{itemize}

==> assets/results/maab_run1.tex <==
\begin{table}[ht]
\centering
\small
\caption{Performance comparison across ML agents and $^{\star}$ablation configurations on diverse datasets. Colorful icons indicate data modality (\texticon: text, \tabularicon: tabular, \imageicon: image, \docicon: document) and problem type (\binclassicon: binary classification, \multiclassicon: multiclass classification, \regressicon: regression, \forecasticon: forecasting, \segmenticon: semantic segmentation, \retrievalicon: retrieval, \multilabelicon: Multi Label Classification). $\uparrow$($\downarrow$) indicates higher(lower) is better. $^\dagger$ columns are not agents, including \modelname's optimal performance with current ML tools to compare with human performance reported in recent literature. \textbf{Bold} numbers indicates best ML agent performance with comparable default configurations.}
\setlength{\tabcolsep}{3.5pt}
\scalebox{0.75}{
\begin{tabular}{p{3cm}|*{5}{>{\centering\arraybackslash}p{1.0cm}@{}}|*{2}{>{\centering\arraybackslash}p{1cm}@{}}|*{2}{>{\centering\arraybackslash}p{1cm}@{}}|*{2}{>{\centering\arraybackslash}p{1cm}@{}}|>{\centering\arraybackslash}p{1cm}@{}|>{\centering\arraybackslash}p{1.5cm}}
\toprule
 \hspace{2cm}\textbf{Agent} & \multicolumn{5}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{}} & \textbf{} & \textbf{} \\
 & \multicolumn{5}{c|}{\textbf{\modelname (ours)}} & \multicolumn{2}{c|}{\textbf{Codex CLI}} & \multicolumn{2}{c|}{\textbf{AIDE}} & \multicolumn{2}{c|}{\textbf{DS-Agent}} & \textbf{AK} & \textbf{Human} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14}
\textbf{Dataset} & \textbf{def} & \textbf{8B$^*$} & \textbf{-ext$^*$} & \textbf{-epi$^*$} & \textbf{24hrs$^\dagger$} & \textbf{def} & \textbf{+rea$^*$} & \textbf{def} & \textbf{+ext$^*$} & \textbf{def} & \textbf{zero-shot} & \textbf{def} & \textbf{Reported$^\dagger$} \\
\midrule
abalone \tabularicon\regressicon$\downarrow$ & \textbf{2.13} & 2.09 & 2.22 & 2.13 & 2.08 & $\times$ & 2.23 & 2.18 & 2.19 & 2.23 & 2.36 & $\times$ & $\times$ \\
airbnb \texticon\tabularicon\multiclassicon$\uparrow$ & \textbf{0.43} & $\times$ & 0.40 & 0.42 & 0.45 & $\times$ & 0.38 & $\times$ & 0.42 & $\times$ & $\times$ & 0.25 & $\times$ \\
airlines \tabularicon\binclassicon$\uparrow$ & \textbf{0.66} & 0.66 & 0.64 & 0.66 & 0.66 & $\times$ & 0.65 & $\times$ & $\times$ & $\times$ & 0.61 & $\times$ & $\times$ \\
bio \tabularicon\binclassicon$\uparrow$ & 0.80 & 0.80 & 0.88 & 0.80 & 0.82 & 0.79 & 0.88 & \textbf{0.87} & 0.88 & 0.79 & 0.79 & $\times$ & $\times$ \\
camoseg \imageicon\segmenticon$\uparrow$ & \textbf{0.83} & $\times$ & $\times$ & 0.84 & 0.85 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.89 \\
cd18 \imageicon\tabularicon\regressicon$\uparrow$ & \textbf{0.45} & $\times$ & -0.63 & 0.45 & 0.15 & -0.41 & -1.29 & $\times$ & 0.24 & -1.94 & 0.33 & -1.84 & -1.84 \\
climate \texticon\retrievalicon$\uparrow$ & \textbf{0.48} & $\times$ & $\times$ & $\times$ & 0.48 & $\times$ & 0.12 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
covertype \tabularicon\multiclassicon$\uparrow$ & \textbf{0.98} & 0.97 & 0.89 & 0.98 & 0.98 & $\times$ & 0.96 & $\times$ & 0.74 & 0.96 & 0.95 & $\times$ & $\times$ \\
electric(H) \tabularicon\forecasticon$\downarrow$ & \textbf{1.44} & $\times$ & 1.75 & 1.41 & 1.30 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 1.23 \\
flood \imageicon\binclassicon$\uparrow$ & 0.68 & $\times$ & 0.58 & 0.68 & 0.80 & $\times$ & 0.44 & \textbf{0.72} & 0.70 & $\times$ & $\times$ & $\times$ & 0.79 \\
fiqa \texticon\retrievalicon$\uparrow$ & \textbf{0.48} & $\times$ & $\times$ & 0.38 & 0.48 & $\times$ & 0.20 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.78 \\
gnad10 \texticon\multiclassicon$\uparrow$ & \textbf{0.84} & 0.84 & 0.88 & 0.84 & 0.89 & $\times$ & 0.85 & $\times$ & $\times$ & $\times$ & 0.69 & $\times$ & 0.90 \\
ham10000 \imageicon\tabularicon\multiclassicon$\uparrow$ & 0.56 & $\times$ & 0.67 & $\times$ & 0.56 & $\times$ & 0.51 & \textbf{0.81} & 0.78 & $\times$ & $\times$ & $\times$ & 0.61 \\
hateful \texticon\imageicon\binclassicon$\uparrow$ & \textbf{0.57} & 0.53 & 0.38 & 0.57 & 0.61 & 0.48 & 0.57 & 0.56 & 0.52 & $\times$ & $\times$ & 0.34 & 0.60 \\
isic2017 \imageicon\segmenticon$\uparrow$ & \textbf{0.75} & $\times$ & $\times$ & $\times$ & 0.76 & $\times$ & 0.11 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.78 \\
funding \texticon\tabularicon\binclassicon$\uparrow$ & \textbf{0.44} & 0.47 & 0.44 & 0.44 & 0.51 & $\times$ & 0.36 & $\times$ & 0.44 & $\times$ & $\times$ & $\times$ & 0.61 \\
memotion \scalebox{0.8}{\texticon\imageicon\tabularicon\multilabelicon}$\uparrow$ & \textbf{0.50} & $\times$ & $\times$ & $\times$ & 0.56 & $\times$ & $\times$ & 0.47 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
mldoc \texticon\multiclassicon$\uparrow$ & \textbf{0.96} & 0.95 & 0.96 & 0.95 & 0.97 & $\times$ & 0.93 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
nn5(D) \tabularicon\forecasticon$\downarrow$ & \textbf{0.76} & $\times$ & $\times$ & 0.76 & 0.79 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.76 \\
petfinder\scalebox{0.9}{\texticon\imageicon\tabularicon\multiclassicon}$\uparrow$ & \textbf{0.39} & 0.39 & 0.36 & 0.39 & 0.41 & $\times$ & 0.40 & $\times$ & 0.38 & 0.35 & 0.39 & 0.39 & 0.41 \\
roadseg \imageicon\segmenticon$\uparrow$ & \textbf{0.47} & $\times$ & $\times$ & $\times$ & 0.47 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.62 \\
rvlcdip \docicon\multiclassicon$\uparrow$ & \textbf{0.87} & $\times$ & 0.89 & 0.87 & 0.92 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
solar(10m) \tabularicon\forecasticon$\downarrow$ & 2.27 & $\times$ & $\times$ & 1.29 & 0.18 & $\times$ & $\times$ & \textbf{1.05} & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
clothing \texticon\tabularicon\regressicon$\uparrow$ & \textbf{0.75} & $\times$ & 0.62 & 0.75 & 0.77 & $\times$ & 0.42 & $\times$ & 0.75 & $\times$ & $\times$ & $\times$ & 0.74 \\
yolanda \tabularicon\regressicon$\downarrow$ & \textbf{8.53} & 8.53 & 8.89 & 8.53 & 8.18 & $\times$ & 9.10 & $\times$ & 8.54 & 1490.6 & $\times$ & $\times$ & $\times$ \\
\midrule
\rowcolor{lightgray}
\textbf{Avg. Rank} & \textbf{2.32} & \textbf{5.98} & \textbf{5.22} & \textbf{3.50} & \textbf{N/A} & \textbf{8.14} & \textbf{4.80} & \textbf{6.70} & \textbf{5.88} & \textbf{7.48} & \textbf{7.94} & \textbf{8.04} & \textbf{N/A} \\
\rowcolor{lightgray}
\textbf{Rel. Time} & \textbf{1.0} & \textbf{} & \textbf{} & \textbf{} & \textbf{N/A} & \textbf{N/A} & \textbf{N/A} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{N/A} \\
\rowcolor{lightgray}
\textbf{Success} & \textbf{100\%} & \textbf{40\%} & \textbf{68\%} & \textbf{80\%} & \textbf{N/A} & \textbf{12\%} & \textbf{72\%} & \textbf{28\%} & \textbf{48\%} & \textbf{24\%} & \textbf{28\%} & \textbf{16\%} & \textbf{N/A} \\
\bottomrule
\end{tabular}
}
\end{table}


% before removing -ext and rename -ext +env to -ext
\iffalse
\begin{table}[ht]
\centering
\small
\caption{Performance comparison across automated machine learning systems and experimental settings on diverse datasets. Colorful icons indicate data modality (\texticon: text, \tabularicon: tabular, \imageicon: image, \docicon: document) and problem type (\binclassicon: binary classification, \multiclassicon: multiclass classification, \regressicon: regression, \forecasticon: forecasting, \segmenticon: semantic segmentation, \retrievalicon: retrieval, \multilabelicon: Multi Label Classification). Metrics are shown with $\uparrow$ indicating higher is better and $\downarrow$ indicating lower is better. Oracle column reports human expert ground truth performance established from recent literature.}

\setlength{\tabcolsep}{3.5pt}
\scalebox{0.75}{
\begin{tabular}{p{3cm}|*{6}{>{\centering\arraybackslash}p{1.0cm}@{}}|*{1}{>{\centering\arraybackslash}p{1.5cm}@{}}|*{2}{>{\centering\arraybackslash}p{1cm}@{}}|*{2}{>{\centering\arraybackslash}p{1cm}@{}}|>{\centering\arraybackslash}p{1cm}@{}|>{\centering\arraybackslash}p{1.5cm}}
\toprule
 \hspace{2cm}\textbf{Agent} & \multicolumn{6}{c|}{\textbf{End-to-End}} & \multicolumn{1}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{End-to-End}} & \multicolumn{2}{c|}{\textbf{}} & \textbf{} & \textbf{} \\
 & \multicolumn{6}{c|}{\textbf{\modelname (ours)}} & \multicolumn{1}{c|}{\textbf{Codex CLI}} & \multicolumn{2}{c|}{\textbf{AIDE}} & \multicolumn{2}{c|}{\textbf{DS-Agent}} & \textbf{AK} & \textbf{Human} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-13} \cmidrule(lr){14-14}
\textbf{Dataset} & \textbf{def} & \textbf{8B} & \textbf{-ext} & \textbf{-ext +env} & \textbf{-epi} & \textbf{24hrs} & \textbf{+rea} & \textbf{def} & \textbf{+ext} & \textbf{def} & \textbf{zero-shot} & \textbf{def} & \textbf{Reported} \\
\midrule
abalone \tabularicon\regressicon$\downarrow$ & 2.13 & 2.09 & 2.22 & 2.22 & 2.13 & 2.08 & 2.23 & 2.18 & 2.19 & 2.23 & 2.36 & $\times$ & $\times$ \\
airbnb \texticon\tabularicon\multiclassicon$\uparrow$ & 0.43 & $\times$ & 0.39 & 0.40 & 0.42 & 0.45 & 0.38 & $\times$ & 0.42 & $\times$ & $\times$ & 0.25 & $\times$ \\
airlines \tabularicon\binclassicon$\uparrow$ & 0.66 & 0.66 & 0.64 & 0.64 & 0.66 & 0.66 & 0.65 & $\times$ & $\times$ & $\times$ & 0.61 & $\times$ & $\times$ \\
bio \tabularicon\binclassicon$\uparrow$ & 0.80 & 0.80 & 0.88 & 0.88 & 0.80 & 0.82 & 0.88 & 0.87 & 0.88 & 0.79 & 0.79 & $\times$ & $\times$ \\
camoseg \imageicon\segmenticon$\uparrow$ & 0.83 & $\times$ & $\times$ & $\times$ & 0.84 & 0.85 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.89 \\
cd18 \imageicon\tabularicon\regressicon$\uparrow$ & 0.45 & $\times$ & -0.28 & -0.63 & 0.45 & 0.15 & -1.29 & $\times$ & 0.24 & -1.94 & 0.33 & -1.84 & -1.84 \\
climate \texticon\retrievalicon$\uparrow$ & 0.48 & $\times$ & $\times$ & $\times$ & $\times$ & 0.48 & 0.12 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
covertype \tabularicon\multiclassicon$\uparrow$ & 0.98 & 0.97 & $\times$ & 0.89 & 0.98 & 0.98 & 0.96 & $\times$ & 0.74 & 0.96 & 0.95 & $\times$ & $\times$ \\
electric(H) \tabularicon\forecasticon$\downarrow$ & 1.44 & $\times$ & $\times$ & 1.75 & 1.41 & 1.30 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 1.23 \\
flood \imageicon\binclassicon$\uparrow$ & 0.68 & $\times$ & 0.68 & 0.58 & 0.68 & 0.80 & 0.44 & 0.72 & 0.70 & $\times$ & $\times$ & $\times$ & 0.79 \\
fiqa \texticon\retrievalicon$\uparrow$ & 0.48 & $\times$ & $\times$ & $\times$ & 0.38 & 0.48 & 0.20 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.78 \\
gnad10 \texticon\multiclassicon$\uparrow$ & 0.84 & 0.84 & 0.87 & 0.88 & 0.84 & 0.89 & 0.85 & $\times$ & $\times$ & $\times$ & 0.69 & $\times$ & 0.90 \\
ham10000 \imageicon\tabularicon\multiclassicon$\uparrow$ & 0.56 & $\times$ & $\times$ & 0.67 & $\times$ & 0.56 & 0.51 & 0.81 & 0.78 & $\times$ & $\times$ & $\times$ & 0.61 \\
hateful \texticon\imageicon\binclassicon$\uparrow$ & 0.57 & 0.53 & $\times$ & 0.38 & 0.57 & 0.61 & 0.57 & 0.56 & 0.52 & $\times$ & $\times$ & 0.34 & 0.60 \\
isic2017 \imageicon\segmenticon$\uparrow$ & 0.75 & $\times$ & $\times$ & $\times$ & $\times$ & 0.76 & 0.11 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.78 \\
funding \texticon\tabularicon\binclassicon$\uparrow$ & 0.44 & 0.47 & 0.43 & 0.44 & 0.44 & 0.51 & 0.36 & $\times$ & 0.44 & $\times$ & $\times$ & $\times$ & 0.61 \\
memotion \scalebox{0.8}{\texticon\imageicon\tabularicon\multilabelicon}$\uparrow$ & 0.50 & $\times$ & $\times$ & $\times$ & $\times$ & 0.56 & $\times$ & 0.47 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
mldoc \texticon\multiclassicon$\uparrow$ & 0.96 & 0.95 & 0.96 & 0.96 & 0.95 & 0.97 & 0.93 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
nn5(D) \tabularicon\forecasticon$\downarrow$ & 0.76 & $\times$ & $\times$ & $\times$ & 0.76 & 0.79 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.76 \\
petfinder\scalebox{0.9}{\texticon\imageicon\tabularicon\multiclassicon}$\uparrow$ & 0.39 & 0.39 & 0.40 & 0.36 & 0.39 & 0.41 & 0.40 & $\times$ & 0.38 & 0.35 & 0.39 & 0.39 & 0.41 \\
roadseg \imageicon\segmenticon$\uparrow$ & 0.47 & $\times$ & $\times$ & $\times$ & $\times$ & 0.47 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & 0.62 \\
rvlcdip \docicon\multiclassicon$\uparrow$ & 0.87 & $\times$ & $\times$ & 0.89 & 0.87 & 0.92 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
solar(10m) \tabularicon\forecasticon$\downarrow$ & 2.27 & $\times$ & $\times$ & $\times$ & 1.29 & 0.18 & $\times$ & 1.05 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\
clothing \texticon\tabularicon\regressicon$\uparrow$ & 0.75 & $\times$ & 0.61 & 0.62 & 0.75 & 0.77 & 0.42 & $\times$ & 0.75 & $\times$ & $\times$ & $\times$ & 0.74 \\
yolanda \tabularicon\regressicon$\downarrow$ & 8.53 & 8.53 & 8.92 & 8.89 & 8.53 & 8.18 & 9.10 & $\times$ & 8.54 & 1490.6 & $\times$ & $\times$ & $\times$ \\
\midrule
\rowcolor{lightgray}
\textbf{Avg. Rank} & \textbf{2.48} & \textbf{6.20} & \textbf{6.08} & \textbf{5.34} & \textbf{3.68} & \textbf{N/A} & \textbf{5.12} & \textbf{6.90} & \textbf{6.00} & \textbf{8.20} & \textbf{7.76} & \textbf{8.24} & \textbf{N/A} \\
\rowcolor{lightgray}
\textbf{Rel. Time} & \textbf{1.0} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{N/A} & \textbf{N/A} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{N/A} \\
\rowcolor{lightgray}
\textbf{Success} & \textbf{100\%} & \textbf{40\%} & \textbf{48\%} & \textbf{68\%} & \textbf{80\%} & \textbf{N/A} & \textbf{72\%} & \textbf{28\%} & \textbf{48\%} & \textbf{24\%} & \textbf{28\%} & \textbf{16\%} & \textbf{N/A} \\
\bottomrule
\end{tabular}
}
\label{tab:main_result}
\end{table}
\fi


==> sections/6_broader_impact.tex <==
\pagebreak
\section*{Broader Impact Statement}
% The 9 pages allocated for the main paper must include a broader impact
% statement regarding the approach, datasets and applications proposed/used in
% your paper. It should reflect on the environmental, ethical and societal
% implications of your work. The statement should require at most one page and
% must be included both at submission and camera-ready time.
%
% If authors have reflected on their work and determined that there are no
% likely negative broader impacts, they may use the following statement:
%
% After careful reflection, the authors have determined that this work presents
% no notable negative impacts to society or the environment.
%
% This section is included in the template as a default, but you can also place these
% discussions anywhere else in the main paper, e.g., in the introduction/future work.
%
% The Centre for the Governance of AI has written an excellent guide for writing
% good broader impact statements (for the NeurIPS conference) that may be a
% useful resource for AutoML-Conf authors:
%
% https://medium.com/@GovAI/a-guide-to-writing-the-neurips-impact-statement-4293b723f832


While our system may improve accessibility and efficiency for researchers and practitioners, we acknowledge potential implications. Automated ML systems could reduce the need for specialized data scientists in some contexts, potentially impacting employment patterns. Additionally, as with any automation technology, there is risk of reinforcing biases present in training data if users deploy solutions without appropriate oversight. The environmental impact of running multiple iterations with large language models warrants consideration, though our approach's improved efficiency may partially mitigate this concern. We believe the potential benefits of expanding access to sophisticated ML techniques across diverse domains outweigh these considerations, particularly for resource-constrained organizations and researchers in underrepresented communities. We encourage users to apply appropriate validation procedures and maintain human oversight when deploying solutions generated by \modelname in sensitive domains.

